Maximum Likelihood Estimation of Differentiated Products Demand Systems

We discuss estimation of the differentiated products demand system of Berry et al (1995) (BLP) by maximum likelihood estimation (MLE). We derive the maximum likelihood estimator in the case where prices are endogenously generated by firms that set prices in Bertrand-Nash equilibrium. In Monte Carlo simulations the MLE estimator outperforms the best-practice GMM estimator on both bias and mean squared error when the model is correctly specified. This remains true under some forms of misspecification. In our simulations, the coverage of the ML estimator is close to its nominal level, whereas the GMM estimator tends to under-cover. We conclude the paper by estimating BLP on the car data used in the original Berry et al (1995) paper, obtaining similar estimates with considerably tighter standard errors.

==> tables/blp95_estimates.tex <==
\begin{tabular}{l|rrrr}
& \textbf{\shortstack{BLP\\\\95}} & \textbf{\shortstack{AGS\\\\'17}} & \textbf{\shortstack{PyBLP\\\\'20}} & \textbf{\shortstack{MLE}}\\\hline
\textbf{alpha price} & 43.501 & 42.870 & 45.898 & 45.227\\
\textbf{sigma const} & 3.612 & 2.522 & 2.962 & 1.924\\
\textbf{sigma hpwt} & 4.628 & 3.525 & 1.388 & 4.611\\
\textbf{sigma air} & 1.818 & 4.167 & 1.424 & 1.991\\
\textbf{sigma mpd} & 1.050 & 0.393 & 0.072 & 0.299\\
\textbf{sigma space} & 2.056 & 1.937 & 0.231 & 2.168\\
\textbf{demand const} & -7.061 & -7.728 & -6.679 & -5.439\\
\textbf{demand hpwt} & 2.883 & 4.620 & 2.774 & 3.175\\
\textbf{demand air} & 1.521 & -1.227 & 0.572 & 0.385\\
\textbf{demand mpd} & -0.122 & 0.293 & 0.340 & 0.086\\
\textbf{demand space} & 3.460 & 3.992 & 3.920 & 3.327\\
\textbf{supply const} & 0.952 & 2.751 & 2.780 & 2.327\\
\textbf{supply loghpwt} & 0.477 & 0.812 & 0.731 & 0.495\\
\textbf{supply air} & 0.619 & 0.430 & 0.528 & 0.601\\
\textbf{supply logmpg} & -0.415 & -0.610 & -0.651 & -0.377\\
\textbf{supply logspace} & -0.046 & -0.352 & -0.472 & 0.028\\
\textbf{supply trend} & 0.019 & 0.027 & 0.018 & 0.015\\
\end{tabular}


==> tables/blp95_estimates_with_se.tex <==
\begin{tabular}{l|rrrr}
& \textbf{\shortstack{BLP}} & \textbf{\shortstack{AGS}} & \textbf{\shortstack{PyBLP}} & \textbf{\shortstack{MLE}}\\\hline
\textbf{alpha price} & 43.501 & 42.870 & 45.898 & 45.227\\
 & (6.43) & (5.56) & (11.75) & (0.77)\\
\textbf{sigma const} & 3.612 & 2.522 & 2.962 & 1.924\\
 & (1.49) & (2.54) & (1.64) & (0.16)\\
\textbf{sigma hpwt} & 4.628 & 3.525 & 1.388 & 4.611\\
 & (1.89) & (2.84) & (2.11) & (0.28)\\
\textbf{sigma air} & 1.818 & 4.167 & 1.424 & 1.991\\
 & (1.70) & (1.41) & (0.43) & (0.23)\\
\textbf{sigma mpd} & 1.050 & 0.393 & 0.072 & 0.299\\
 & (0.27) & (0.28) & (1.00) & (0.04)\\
\textbf{sigma space} & 2.056 & 1.937 & 0.231 & 2.168\\
 & (0.58) & (0.60) & (3.84) & (0.11)\\
\textbf{demand const} & -7.061 & -7.728 & -6.679 & -5.439\\
 & (0.94) & (1.16) & (1.30) & (0.33)\\
\textbf{demand hpwt} & 2.883 & 4.620 & 2.774 & 3.175\\
 & (2.02) & (1.13) & (0.83) & (0.35)\\
\textbf{demand air} & 1.521 & -1.227 & 0.572 & 0.385\\
 & (0.89) & (1.38) & (0.35) & (0.16)\\
\textbf{demand mpd} & -0.122 & 0.293 & 0.340 & 0.086\\
 & (0.32) & (0.16) & (0.10) & (0.06)\\
\textbf{demand space} & 3.460 & 3.992 & 3.920 & 3.327\\
 & (0.61) & (0.35) & (0.32) & (0.17)\\
\textbf{supply const} & 0.952 & 2.751 & 2.780 & 2.327\\
 & (0.19) & (0.08) & (0.10) & (0.04)\\
\textbf{supply loghpwt} & 0.477 & 0.812 & 0.731 & 0.495\\
 & (0.06) & (0.06) & (0.07) & (0.03)\\
\textbf{supply air} & 0.619 & 0.430 & 0.528 & 0.601\\
 & (0.04) & (0.05) & (0.04) & (0.02)\\
\textbf{supply logmpg} & -0.415 & -0.610 & -0.651 & -0.377\\
 & (0.06) & (0.05) & (0.07) & (0.04)\\
\textbf{supply logspace} & -0.046 & -0.352 & -0.472 & 0.028\\
 & (0.08) & (0.11) & (0.12) & (0.06)\\
\textbf{supply trend} & 0.019 & 0.027 & 0.018 & 0.015\\
 & (0.00) & (0.00) & (0.00) & (0.00)\\
\end{tabular}


==> tables/blp95_se_estimates.tex <==
\begin{tabular}{l|rrrr}
& \textbf{\shortstack{BLP\\\\95}} & \textbf{\shortstack{AGS\\\\'17}} & \textbf{\shortstack{PyBLP\\\\'20}} & \textbf{\shortstack{MLE}}\\\hline
\textbf{alpha price} & 6.427 & 5.558 & 11.748 & 0.769\\
\textbf{sigma const} & 1.485 & 2.537 & 1.637 & 0.158\\
\textbf{sigma hpwt} & 1.885 & 2.844 & 2.107 & 0.278\\
\textbf{sigma air} & 1.695 & 1.414 & 0.435 & 0.229\\
\textbf{sigma mpd} & 0.272 & 0.281 & 1.002 & 0.045\\
\textbf{sigma space} & 0.585 & 0.596 & 3.837 & 0.113\\
\textbf{demand const} & 0.941 & 1.156 & 1.304 & 0.327\\
\textbf{demand hpwt} & 2.019 & 1.129 & 0.833 & 0.346\\
\textbf{demand air} & 0.891 & 1.382 & 0.349 & 0.161\\
\textbf{demand mpd} & 0.320 & 0.157 & 0.098 & 0.056\\
\textbf{demand space} & 0.610 & 0.354 & 0.322 & 0.168\\
\textbf{supply const} & 0.194 & 0.084 & 0.104 & 0.039\\
\textbf{supply loghpwt} & 0.056 & 0.060 & 0.071 & 0.030\\
\textbf{supply air} & 0.038 & 0.053 & 0.040 & 0.019\\
\textbf{supply logmpg} & 0.055 & 0.049 & 0.071 & 0.041\\
\textbf{supply logspace} & 0.081 & 0.110 & 0.125 & 0.055\\
\textbf{supply trend} & 0.002 & 0.002 & 0.002 & 0.001\\
\end{tabular}


==> tables/mean_bias_summary.tex <==
\begin{tabular}{lcccccc}
\toprule
&\multicolumn{3}{c}{GMM}&\multicolumn{3}{c}{MLE}\\
\cmidrule(lr){2-4}
\cmidrule(lr){5-7}
& $\alpha$ & $\sigma_{x}$ & $\sigma_{price}$ & $\alpha$ & $\sigma_{x}$ & $\sigma_{price}$\\
\midrule  
\textbf{No covariance} & 0.1201 & -0.0947 & 0.0271 & 0.0338 & 0.0067 & -0.0161\\\addlinespace[5pt]
\textbf{Low covariance} & 0.0971 & -0.0439 & 0.0128 & 0.0335 & 0.0106 & -0.0239\\\addlinespace[5pt]
\textbf{High covariance} & 0.0394 & -0.0763 & 0.0089 & 0.0500 & -0.0040 & -0.0293\\\addlinespace[5pt]
\textbf{Laplace, no covariance} & 0.1131 & -0.0815 & 0.0209 & 0.0331 & -0.0039 & -0.0139\\\addlinespace[5pt]
\textbf{Laplace, low covariance} & 0.0761 & -0.0601 & 0.0159 & 0.0488 & 0.0034 & -0.0204\\\addlinespace[5pt]
\textbf{Supply misspecification} & 0.1998 & 0.0752 & -0.0064 & 0.9448 & 0.3040 & -0.0469\\\addlinespace[5pt]
\textbf{Ownership misspecification} & -0.0456 & -0.1984 & 0.0344 & -0.0030 & -0.0905 & -0.0209\\
\bottomrule
\end{tabular}


==> tables/mean_se.tex <==
\begin{tabular}{lcccccc}
\toprule
&\multicolumn{3}{c}{GMM}&\multicolumn{3}{c}{MLE}\\
\cmidrule(lr){2-4}
\cmidrule(lr){5-7}
& $\alpha$ & $\sigma_{x}$ & $\sigma_{price}$ & $\alpha$ & $\sigma_{x}$ & $\sigma_{price}$\\
\midrule  
\textbf{No covariance} & 0.2973 & 0.3036 & 0.1275 & 0.1962 & 0.2163 & 0.1244\\\addlinespace[5pt]
\textbf{Low covariance} & 0.2818 & 0.2723 & 0.2152 & 0.2271 & 0.1926 & 0.1225\\\addlinespace[5pt]
\textbf{High covariance} & 0.2829 & 0.2884 & 0.1597 & 0.2999 & 0.2014 & 0.1363\\\addlinespace[5pt]
\textbf{Laplace, no covariance} & 0.3029 & 0.3200 & 0.1376 & 0.2041 & 0.2234 & 0.1269\\\addlinespace[5pt]
\textbf{Laplace, low covariance} & 0.2843 & 0.2787 & 0.1457 & 0.2476 & 0.2009 & 0.1256\\\addlinespace[5pt]
\textbf{Supply misspecification} & 0.2868 & 0.3022 & 0.1622 & 0.1989 & 0.2106 & 0.1042\\\addlinespace[5pt]
\textbf{Ownership misspecification} & 0.2644 & 0.2403 & 0.1040 & 0.2971 & 0.1892 & 0.1254\\
\bottomrule
\end{tabular}


==> tables/percent_in_ci.tex <==
\begin{tabular}{lcccccc}
\toprule
&\multicolumn{3}{c}{GMM}&\multicolumn{3}{c}{MLE}\\
\cmidrule(lr){2-4}
\cmidrule(lr){5-7}
& $\alpha$ & $\sigma_{x}$ & $\sigma_{price}$ & $\alpha$ & $\sigma_{x}$ & $\sigma_{price}$\\
\midrule    
% & \textbf{\shortstack{GMM\\\\$\alpha$}} & \textbf{\shortstack{GMM\\\\$\sigma_{x}$}} & \textbf{\shortstack{GMM\\\\$\sigma_{price}$}} & \textbf{\shortstack{MLE\\\\$\alpha$}} & \textbf{\shortstack{MLE\\\\$\sigma_{x}$}} & \textbf{\shortstack{MLE\\\\$\sigma_{price}$}}\\\hline
\textbf{No covariance} & 0.8570 & 0.9220 & 0.7930 & 0.9450 & 0.9330 & 0.9440\\\addlinespace[5pt]
\textbf{Low covariance} & 0.8890 & 0.9510 & 0.7700 & 0.9250 & 0.9390 & 0.9370\\\addlinespace[5pt]
\textbf{High covariance} & 0.8400 & 0.9310 & 0.7210 & 0.8760 & 0.9450 & 0.9550\\\addlinespace[5pt]
\textbf{Laplace, no covariance} & 0.8600 & 0.9340 & 0.7910 & 0.9430 & 0.9500 & 0.9190\\\addlinespace[5pt]
\textbf{Laplace, low covariance} & 0.8830 & 0.9480 & 0.7720 & 0.9070 & 0.9380 & 0.9030\\\addlinespace[5pt]
\textbf{Supply misspecification} & 0.9263 & 0.9687 & 0.6983 & 0.0131 & 0.6408 & 0.8648\\\addlinespace[5pt]
\textbf{Ownership misspecification} & 0.8280 & 0.8080 & 0.7960 & 0.8940 & 0.9070 & 0.9250\\
\bottomrule
\end{tabular}


==> tables/rmse_summary.tex <==
\begin{tabular}{lcccccc}
\toprule
&\multicolumn{3}{c}{GMM}&\multicolumn{3}{c}{MLE}\\
\cmidrule(lr){2-4}
\cmidrule(lr){5-7}
& $\alpha$ & $\sigma_{x}$ & $\sigma_{price}$ & $\alpha$ & $\sigma_{x}$ & $\sigma_{price}$\\
\midrule  
\textbf{No covariance} & 0.4247 & 0.3371 & 0.1259 & 0.1969 & 0.2252 & 0.1032\\\addlinespace[5pt]
\textbf{Low covariance} & 0.4123 & 0.2687 & 0.1282 & 0.2833 & 0.2018 & 0.1098\\\addlinespace[5pt]
\textbf{High covariance} & 0.4014 & 0.2901 & 0.1408 & 0.4309 & 0.2038 & 0.1105\\\addlinespace[5pt]
\textbf{Laplace, no covariance} & 0.4567 & 0.3422 & 0.1273 & 0.2151 & 0.2250 & 0.1099\\\addlinespace[5pt]
\textbf{Laplace, low covariance} & 0.3755 & 0.2726 & 0.1289 & 0.3253 & 0.2054 & 0.1150\\\addlinespace[5pt]
\textbf{Supply misspecification} & 0.4168 & 0.3176 & 0.1372 & 0.9856 & 0.4059 & 0.1261\\\addlinespace[5pt]
\textbf{Ownership misspecification} & 0.3904 & 0.3213 & 0.1178 & 0.3450 & 0.2149 & 0.1081\\
\bottomrule
\end{tabular}

